A Nice Labelling for Tree-Like Event Structures of Degree 3 (Extended Version)

We address the problem of finding nice labellings for event structures of degree 3. We develop a minimum theory by which we prove that the labelling number of an event structure of degree 3 is bounded by a linear function of the height. The main theorem we present in this paper states that event structures of degree 3 whose causality order is a tree have a nice labelling with 3 colors. Finally, we exemplify how to use this theorem to construct upper bounds for the labelling number of other event structures of degree 3.

==> macros.tex <==
\RequirePackage{ifthen}
\RequirePackage{MnSymbol}

%% Hacks, overwrite
\newlength{\mylength}
\newlength{\mylengthu}
\newlength{\mylengthd}
% \newcommand{\overwrite}[2]{%
% \settowidth{\mylength}{\mbox{$#1$}}%
% #1\hspace{-\mylength}#2%
% }
\newcommand{\overwrite}[2]{%
\settowidth{\mylengthu}{\mbox{$#1$}}%
\settowidth{\mylengthd}{\mbox{$#2$}}%
\ifthenelse{\lengthtest{\mylengthu >\mylengthd}}%
{#1\hspace{-\mylengthu}\parbox{\mylengthu}{\myhfill$#2$\myhfill}}%
{#2\hspace{-\mylengthd}\parbox{\mylengthd}{\myhfill$#1$\myhfill}}%
}

%% \cal not defined in elsart ????
%\newcommand{\cal}[1]{\mathcal{#1}}

%% Spacing
\newcommand{\breath}{\vskip 6pt}
\newcommand{\takebreath}{\vskip -4pt}
\newcommand{\proofbreath}{\newline\noindent\mbox{\hspace{12pt}}}

\newcommand{\myhfill}{\mbox{\hspace{0mm}}\hfill\mbox{\hspace{0mm}}}

%% Theorems
\newcommand{\eproofofclaim}{\mbox{\hspace{10mm}}\hfill\mbox{$\Box$\hspace{2mm}\emph{Claim}}\par\breath}

%% General
\newcommand{\set}[1]{\{\,#1\,\}}
\newcommand{\couple}[1]{\{#1\}}
\newcommand{\card}[1]{\mathrm{card}#1}
\newcommand{\N}{\mathbb{N}}
\newcommand{\mymod}{\,\mathrm{mod}\,}

%% Particular
%\newcommand{\CYf}{\mathcal{SC}_{\geq 4}}
\newcommand{\CYf}{\mathtt{SC}_{4}}

%% Graphs
\newcommand{\cl}{\omega}
\newcommand{\chr}{\chi}
\newcommand{\nl}{\mathrm{nl}}
\newcommand{\CL}{\mathcal{CL}}

%% Order
\newcommand{\filter}[1]{\uparrow\!\{\,#1\,\}}
\newcommand{\ideal}[1]{\downarrow\!\!\{\,#1\,\}}
\newcommand{\idealof}[1]{\downarrow\!\!#1}
\newcommand{\lcover}{\prec}
\newcommand{\lcovers}{\lcover}
\newcommand{\comp}{\simeq}
\newcommand{\uncomp}{\not\comp}
\newcommand{\ncomp}{\not\comp}
\newcommand{\height}[1][]{\mathrm{h}_{#1}}
\newcommand{\heightp}[1][]{\height[#1]^{\!\!+}}
\newcommand{\width}[1][]{\mathrm{w}}
\newcommand{\fat}{\mathrm{f}}
\newcommand{\lord}{\lhd}

%\newcommand{\deg}{\cl}

%%
%% Event structures
%%
\newcommand{\E}{\mathcal{E}} %% Event structure
\newcommand{\D}{\mathcal{D}} %% Domain
\newcommand{\G}{\mathcal{G}} %% Graph
\newcommand{\CNF}{\mathcal{C}} %% Configurations
\newcommand{\Hi}{\mathcal{H}} %% History-aware configurations
\newcommand{\I}{\mathcal{I}} %% Event structure

\newcommand{\conflict}{\smile}
\newcommand{\confl}{\conflict}
\newcommand{\concurrent}{\frown}
\newcommand{\conc}{\concurrent}
\newcommand{\orthogonal}{\eqfrown}
\newcommand{\orth}{\orthogonal}
\newcommand{\minimalconflict}{\smileeq}
\newcommand{\mconflict}{\minimalconflict}
\newcommand{\mconfl}{\minimalconflict}
\newcommand{\nconc}{\not\conc}
%\newcommand{\weakconcurrent}{\frowneq}
\newcommand{\weakconcurrent}{\,\overwrite{\raisebox{4pt}{$\conc$}}{\raisebox{-1pt}{$\comp$}}\,}
\newcommand{\wconc}{\weakconcurrent}
\newcommand{\north}{\not\orth}
\newcommand{\orthogonalp}{\bowtie^{+}}
\newcommand{\skewn}[1][]{\mathrm{skew}_{#1}}

%% Orderings on sets
\renewcommand{\O}[1][\lord]{\mathtt{N}^{#1}}
\renewcommand{\L}[1][\lord]{\Soc^{#1}}
\newcommand{\B}{\mathtt{B}}
\newcommand{\C}[1][\lord]{\mathtt{B}^{#1}}
\newcommand{\Ld}{\mathcal{L}_{0,2}}
\newcommand{\Lu}{\mathcal{L}_{1}}


\newcommand{\Soc}{\mathtt{S}}
\newcommand{\Fam}{\mathtt{F}}


%%% Logics
% \newcommand{\tand}{\textrm{ and }}
% \newcommand{\timplies}{\textrm{ implies }}
% \newcommand{\tst}{\textrm{ s.t. }}

%% Arrows
\newcommand{\rTo}{\longrightarrow}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "0"
%%% End: 

